Long term optical variability of bright X-ray point sources in elliptical galaxies

We present long term optical variability studies of bright X-ray sources in four nearby elliptical galaxies with {\it Chandra} Advanced CCD Imaging Spectrometer array (ACIS-S) and {\it Hubble Space Telescope (HST)} Advanced Camera for Surveys observations. Out of the 46 bright (X-ray counts $> 60$) sources that are in the common field of view of the {\it Chandra} and {\it HST} observations, 34 of them have potential optical counterparts, while the rest of them are optically dark. After taking into account of systematic errors, estimated using the field optical sources as reference, we find that four of the X-ray sources (three in NGC1399 and one in NGC1427) have variable optical counterparts at a high significance level. The X-ray luminosities of these source are $\sim 10^{38}$ $\rm ergs~s^{-1}$ and are also variable on similar time-scales. The optical variability implies that the optical emission is associated with the X-ray source itself rather than being the integrated light from a host globular cluster. For one source the change in optical magnitude is $> 0.3$, which is one of the highest reported for this class of X-ray sources and this suggests that the optical variability is induced by the X-ray activity. However, the optically variable sources in NGC1399 have been reported to have blue colours ($g - z > 1$). All four sources have been detected in the infra-red (IR) by {\it Spitzer} as point sources, and their ratio of $5.8$ to $3.6 \mu m$ flux are $> 0.63$ indicating that their IR spectra are like those of Active Galactic Nuclei (AGN). While spectroscopic confirmation is required, it is likely that all four sources are background AGNs. We find none of the X-ray sources having optical/IR colours different from AGNs, to be optically variable.

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

